A Four-Pronged Defense Against Byzantine Attacks in Federated Learning

\textit{Federated learning} (FL) is a nascent distributed learning paradigm to train a shared global model without violating users' privacy. FL has been shown to be vulnerable to various Byzantine attacks, where malicious participants could independently or collusively upload well-crafted updates to deteriorate the performance of the global model. However, existing defenses could only mitigate part of Byzantine attacks, without providing an all-sided shield for FL. It is difficult to simply combine them as they rely on totally contradictory assumptions. In this paper, we propose FPD, a \underline{\textbf{f}}our-\underline{\textbf{p}}ronged \underline{\textbf{d}}efense against both non-colluding and colluding Byzantine attacks. Our main idea is to utilize absolute similarity to filter updates rather than relative similarity used in existingI works. To this end, we first propose a reliable client selection strategy to prevent the majority of threats in the bud. Then we design a simple but effective score-based detection method to mitigate colluding attacks. Third, we construct an enhanced spectral-based outlier detector to accurately discard abnormal updates when the training data is \textit{not independent and identically distributed} (non-IID). Finally, we design update denoising to rectify the direction of the slightly noisy but harmful updates. The four sequentially combined modules can effectively reconcile the contradiction in addressing non-colluding and colluding Byzantine attacks. Extensive experiments over three benchmark image classification datasets against four state-of-the-art Byzantine attacks demonstrate that FPD drastically outperforms existing defenses in IID and non-IID scenarios (with $30\%$ improvement on model accuracy).

==> Section/1-introduction.tex <==
\section{INTRODUCTION}


\textit{Federated learning} (FL)~\cite{FedAvg} emerges as a new distributed machine learning paradigm recently, where the training data and the learning process are fully controlled by the clients, thus alleviating the privacy concern. 
%Typically, there are two crucial roles involved in a FL systems, \ie, a central server and several clients (also known as participants). The central server is responsible for broadcasting a global model to the clients and upgrading it with the model updates shared by the clients. The clients train models locally over their private data and then upload the model updates to the central server. FL has earned extensive attention in both academia and industry due to its extraordinary ability to learn a high-quality global model over distributed data and the guarantee on privacy.
However, due to its decentralized nature, FL is found to be highly vulnerable to Byzantine attacks, where malicious participants contribute poisoned updates to damage the global model. Generally, Byzantine attacks can be categorized into non-colluding attacks~\cite{PCA,Zeno} where attackers upload malicious updates independently, and colluding attacks~\cite{ALittleIsEnough,IPM,LocalModelPoisoning,AGRT,MPAF} where attackers share information (\eg, training data, and model updates) to each other and collusively design well-crafted updates. In particular, colluding attackers tend to upload  similar or totally identical updates to avoid being treated as outliers~\cite{SparseFed}.

% Specifically, attackers can construct malicious updates through falsifying the parameters directly (\ie, model poisoning attack)~\cite{ALittleIsEnough,IPM,LocalModelPoisoning,AGRT}, or training models on poisoned data (\ie, data poisoning attack)~\cite{PCA,xie2019dba}. Moreover, the attackers can also collude or not, corresponding to the collusion attack and the dispersion attack respectively.

To defend against these two kinds of attacks, massive defensive schemes have been proposed in recent years. For the non-colluding attacks, existing defenses, such as Krum~\cite{Krum}, FABA~\cite{FABA}, Median~\cite{TrimmedMean}, FedInv~\cite{FedInv}, AFA~\cite{AFA}, manage to remove or circumvent the outliers based on the intuition that benign updates are much similar to each other due to the same optimization objective, while the malicious ones can be considered as outliers. To resist colluding attacks, existing works like \black{FoolsGold~\cite{Sybils}, LOF~\cite{WeightAttack}, and Contra}~\cite{Contra} propose to punish the relatively similar updates by distributing smaller weights in the aggregation stage. Unfortunately, these defenses (or simply combining them) cannot mitigate non-colluding and colluding attacks simultaneously, \black{since the intuitions behind them are almost opposite arguing whether the malicious updates are similar to each other.}




Recent studies like \black{LFR}~\cite{LocalModelPoisoning}, Zeno~\cite{Zeno}, FLTrust~\cite{FLTrust}, DiverseFL~\cite{DiverseFL} attempt to defend against both attacks simultaneously. Instead of relying on the distribution of the updates, they turn to an auxiliary dataset to validate the performance (\eg, loss or accuracy) of each update~\cite{LocalModelPoisoning,Zeno}, or construct a reliable update as a reference~\cite{FLTrust,DiverseFL}. These performance based defenses hold that malicious updates inevitably degrade model performance in a degree. Although performing much better in non-colluding and part of colluding scenarios, these defenses fail to work when malicious updates are slightly noised but harmful (\eg, LIE attack~\cite{ALittleIsEnough}), especially  when the data is \textit{not independent and identically distributed} (non-IID). Moreover, \black{the assumption of possessing an auxiliary dataset will violate users' privacy as they usually require that the auxiliary dataset has the same distribution with the clients' local training datasets.} In summary, an effective defense providing an all-sided shield for FL is still missing yet. 


% These defenses are designed based on one of the following three intuitions. The first intuition is that benign updates may be extremely similar to each other due to the same optimization objective, while the malicious ones can be considered as outliers. In light of this, most of the defenses~\cite{Krum,FABA,TrimmedMean,FedInv,AGRT,AFA} manage to remove or circumvent the outliers. The second intuition is that attackers may also craft more compact malicious updates to bewilder the central server. Based on it, several defenses~\cite{Sybils,WeightAttack,Contra} propose to punish the excessively similar updates by distributing smaller weights to them in the aggregation stage. The last intuition is that malicious updates inevitably degrade model performance. Inspired by this, some defenses turn to an auxiliary dataset to validate the performance (\eg, loss or accuracy) of each update~\cite{LocalModelPoisoning,Zeno}, or construct a reliable update as a reference~\cite{FLTrust,DiverseFL}. For narrative convenience, we call these three types of defenses Type-I, Type-II, and Type-III respectively.


% However, all the existing defenses have the following shortcomings much or less. Firstly, they are fragile to complicated and volatile attack scenarios. For example, the Type-I defense are ineffective in collusion attack scenario, and the Type-II defense drastically punish benign updates in dispersion attack scenario. Secondly, they either ignore or thoughtlessly consider the client selection step, offering more opportunity for attackers to share misleading information. Lastly, they fail to distinguish the slightly noised but harmful updates from benign ones.

To tackle these issues, we propose FPD, a \underline{\textbf{f}}our-\underline{\textbf{p}}ronged \underline{\textbf{d}}efense against both non-colluding and colluding Byzantine attacks. Our main observation is that \black{the contradictory intuitions behind existing two kinds of schemes arises because both of them rely on the   relative similarity between updates due to the lack of a gold standard to evaluate each update in FL. In light of this, we propose to construct an artificial gold standard, which is an empirically determined threshold, to form absolute similarity that can be used to detect colluding attacks. Meanwhile, non-colluding attacks can still be detected based on relative similarity. In this way, the contradictory of solely exploiting relative similarity  can be reconciled naturally. }
Specifically, we propose two defense modules relying on absolute similarity and relative similarity to defend against colluding attacks and non-colluding attacks, respectively. In addition, we design a reliable client selection  strategy to prevent the majority of threats and the update denoising method to  rectify the update directions, in order to further \black{alleviate the impact of colluding attacks}.



In summary, we offer the following contributions:

\begin{itemize}
    \item We propose a new FL defense scheme FPD, which is effective in defending against  non-colluding and colluding Byzantine attacks simultaneously.
    
    \item We propose two novel auxiliary defense modules (\ie, reliable client selection and update denoising) to further enhance the defense ability.
    
    % Specifically, the \textit{reliable client selection} reduces the selected probabilities of those previously poor-performed clients so that only a limited number of attackers have a chance to poison the global model. And the \textit{update denoising} can rectify the direction of the slightly noised but harmful updates.
    
    % \item Unlike existing defenses, which are effective in either collusion attack scenario or dispersion attack scenario, the proposed FPD can deal with both scenarios readily.

    \item We demonstrate the advantage of FPD via extensive experiments on three benchmark datasets against four state-of-the-art attacks. Compared with five distinguished defenses, our scheme achieves the best performance in both IID and non-IID scenarios.
    
\end{itemize}

==> Section/2-relatedwork.tex <==
\section{RELATED WORK}

\subsection{FL in Cross-Modality Medical Image}
Cross-modality medical imaging data refers to medical data collected from different imaging modalities, such as MRI, CT, and PET, among others. It is crucial in modern medicine as it allows medical professionals to obtain highly detailed images of the human body, leading to more accurate diagnoses, effective treatment plans, and improved patient outcomes~\cite{li2020towards,jin2022evaluating}. Its applications are numerous, including identifying and diagnosing cancer~\cite{palmirotta2018liquid}, guiding surgical procedures~\cite{storaas2022explainability}, monitoring treatment progress~\cite{garcia2018mental}, and studying disease progression~\cite{fard2022cnns}. 



One of the main characteristics of cross-modality medical data is that it is heterogeneous in terms of data distribution and amounts in the data-collection process. In FL, this heterogeneity may lead to inferior performance for clients with either less data or a data distribution deviating from others. The heterogeneity of cross-modality medical data may further exacerbate the challenges of data distribution shift and data heterogeneity. In the preprocessing stage, FL algorithms typically require that the data be preprocessed in a standardized way to ensure consistency across different clients. However, due to the heterogeneity of cross-modality medical data, this may not always be feasible. This can result in different clients having different preprocessing procedures, leading to further data heterogeneity.
To address these challenges,~\cite{ahmed2022federated,tan2023transfer} use transfer learning techniques to transfer knowledge learned from one modality to another, thereby reducing the amount of data required for training.~\cite{shyu2021systematic,feki2021federated} propose using data augmentation techniques to increase the amount of data available for training, while~\cite{anderson2017adaptive,zhou2022generalizable} focus on developing novel algorithms that can handle data heterogeneity more effectively.

%Cross-modality medical image fusion is the integration of imaging data from different imaging modalities into a single diagnostic examination to improve diagnostic accuracy and facilitate treatment planning~\cite{survey1,survey2,survey3,survey4}. For instance, PT data fusion combines PET's functional imaging with CT's anatomical imaging into a single diagnostic examination to improve downstream segmentation task~\cite{PT_segmentation,PT_segmentation_1}. 
% Spatial registration-based and automated deep learning-based methods have been proposed, the latter demonstrating significant potential, but requiring multiple complementary sources of heterogeneous information during training, posing significant design challenges for models~\cite{PT_auto,PT_auto_1}. ~\cite{PT_software} proposed a spatial registration-based method commonly used in medical software, which matches different modalities' data directly in terms of spatial location and coordinates. ~\cite{quantitative_PT} explored the quantitative analysis of the impact of different imaging agents on PET and CT images. Other methods, such as bilinear pooling-based fusion\cite{PT_bineal, PT_bineal_1} and attention mechanisms~\cite{PT_attention_1, PT_spatial_attention}, have also been proposed to capture high-order statistical information and explore the interaction between different modalities' images. However, these methods overlook the interaction between shallow and deep features within a single modality, failing to fully utilize available pathological information. To achieve complementary heterogeneous information, Our method aims to design both intra-modality and inter-modality fusion to meet the needs of cross-modality data fusion, which can explicitly improve the downstream segmentation task results on the input end.




\subsection{Fairness-Aware FL} 
% 多模态数据
Machine learning fairness involves examining the unintended behavior of machine learning models, which is a crucial aspect of ensuring equitable and unbiased decision-making~\cite{mehrabi2021survey,caton2020fairness}. Ensuring fairness in FL, a distributed machine learning setting, poses unique challenges given the complexity, heterogeneity, and diversity of client data. In FL, "collaboration fairness" and "performance fairness" are the two primary forms of fairness that are extensively researched~\cite{jiang2023fair}. The former pertains to maintaining equitable participation of all clients in the learning process, without any one client dominating the computation or communication resources~\cite{zhou2021towards,lyu2020collaborative}. The latter, on the other hand, focuses on ensuring that no client or group of clients is disadvantaged by the learned model due to differences in their local data distribution or other factors~\cite{zhang2020fairfl,deng2020distributionally}. 


\begin{figure*}[ht]
\begin{center}
    \centering
    \includegraphics[width=0.9\textwidth]{Section/Figure/mm流程图.pdf}
\caption{\textbf{Analysis workflow.}}
    \label{fig:FedGEM}
\end{center}
\end{figure*}

For collaboration fairness, CGSV~\cite{NEURIPS2021_8682cc30} is a gradient reward mechanism based on the cosine gradient Shapley value to ensure fairness in collaborative machine learning. ~\cite{kang2019incentive} suggested using local computation and communication costs to estimate the contribution of each client. ~\cite{lyu2020collaborative} proposes to use the validation performance of each client to achieve fairness. To address performance fairness, q-FedAvg~\cite{li2019fair} formulates a new optimization objective that is able to control the loss weights of each client during training. ~\cite{mohri2019agnostic} proposed an optimization scheme that aims to improve the performance of the single worst device. However, these efforts rarely balance both collaboration and performance fairness, and the trade-off between fairness and global model performance often leads to sacrificing the latter. In scenarios where high accuracy is required for FL applications (e.g., medical imaging) such costs are undesirable. Therefore, considering the highly heterogeneous and complex nature of client data in real-world medical imaging applications, simultaneously addressing fairness and general model performance amid the need for high accuracy in FL is an ongoing challenge. While cross-modality medical data fusion can improve the accuracy of medical diagnoses. However, it also raises concerns about fairness, as different modalities may contain varying levels of information and unequal representation of certain demographic groups, resulting in biased models. The impact of these fairness issues is significant, and therefore, it is crucial to develop approaches that address them effectively.





%FedCI~\cite{song2019profit} uses a contribution index based on local data and model updates to allocate profits among clients.







==> Section/3-methodology.tex <==
\section{Methods}

\subsection{Overview of CMFL}
% 分别对应着三个挑战是如何解决的思路
In this paper, we introduce CMFL to address performance and collaboration fairness challenges in FL with heterogeneous cross-modal medical data. The workflow of the proposed method is depicted in Fig.~\ref{fig:FedGEM}.


% Assume there is a general FL system, comprising of $N\in \mathbb{N}$ clients and a central server, each client with a local distribution denoted by $\mathcal{D}_i$, forming the set $\mathcal{D}=\bigcup_{i=1}^{N} \mathcal{D}_{i}$. The distribution $\mathcal{D}$ is defined on the space $\mathcal{S}$, where $\mathcal{S}=x \times y$, and $x \in \mathbb{R}^d$ and $y$ denote data input and output respectively. Let $\zeta:=\left\{\nabla_1^{t}, \ldots,\ldots,\nabla_{M}^{t}\right\}$ with size $M$ be the union of local model update $\nabla\in \mathbb{R}^d$ among all clients at communication round $t$, and is drawn from the joint distribution $\mathcal{D}^M$, denoted by $S \sim \mathcal{D}^M$. 

% Assuming a utility function $U$ that maps the sample space $\mathcal{Z}$ to the interval $[0,1]$, we can evaluate the value of any subset $S\subseteq \mathcal{Z}$ as $U(S)$. As an example, in the context of training clients, $U$ is often chosen to represent the accuracy of an empirical risk minimizer. We introduce the notation $\mathrm{SV}$ to represent a specific function defined as follows.




\subsection{Hierarchical Contribution Rectification}


\paragraph{\textbf{Collaboration Rectification}} As for Collaboration Fairness, we simultaneously rectify the valuation in two complementary spaces (i.e., direction and dependence space).  In the direction space, the main purpose is to rectify the difference in gradient direction between the client's gradient and the global gradient.  The dependence space helps to capture the trend of client gradient changes and the correlation between the client's gradient and the overall average gradient.  Considering both spaces ensures that both indicators are represented to some extent.  For instance, it aids in encouraging clients with weaker associations to the average gradient direction to contribute their unique information without compromising the rights of other clients, leading to improved collaboration fairness.

In the dependence space, we quantify the contribution of each client by measuring the optimization dependency of their model gradient $\mathbf{g_{i, t}}$ with respect to the average gradient $\overline{\mathbf{g}_t}$. We calculate the dependence correlation using the reciprocal of the Pearson correlation coefficient as follows:

\begin{equation}
\operatorname{Dep}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_t\right)=\frac{\sqrt{\operatorname{var}\left(\mathbf{g_{i, t}}\right) \cdot \operatorname{var}\left(\overline{\mathbf{g}}_{t}\right)}}{\operatorname{cov}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_{t}\right)}
\end{equation}

A high dependency score close to 1 indicates a strong linear correlation between client i and the average result, meaning that the gradient direction of client i is highly aligned with the average gradient direction. In contrast, a dependency score greater than 1 indicates a weak linear correlation, suggesting that the gradient direction of client i is less aligned with the average gradient direction, potentially indicating that the client may possess new and unique information. After utilizing this method, we can assign higher weights to clients with weak linear correlation. This encourages them to contribute their unique information and promotes collaboration fairness. To avoid unstable score distribution, we use the exponential function to transform the Pearson correlation coefficient to the range of [0,1]. This ensures stable score distribution and improves the robustness of the model on different datasets. We further normalize the transformed values for all clients to ensure the summation over clients adds up to 1. We compute the dependence score, i.e., $w_{i, \text { Dep }}=\exp \left(\operatorname{Dep}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_t\right)\right) / \sum_{i=1}^N \exp \left(\operatorname{Dep}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_t\right)\right)$. 




In the direction space, we rectify each client's contribution to the average model through using cosine similarity between the client's model gradient and the average gradient, i.e., $\operatorname{Dir}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_t\right)=\mathrm{cos\ }\left(\mathbf{g_{i, t}},\overline{\mathbf{g}}_t\right)$.  And we also use the exponential function and normalize the term to ensure the summation over clients  $w_{i, \text { Dir }}=\exp \left(\operatorname{Dir}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_t\right)\right) / \sum_{i=1}^N \exp \left(\operatorname{Dir}\left(\mathbf{g_{i, t}}, \overline{\mathbf{g}}_t\right)\right)$. Finally, we combine the weights of each client in both space by taking the average which ensures that clients with different data distributions are rectified appropriate weights and obtain the weights of each client in collaboration fairness.


\paragraph{\textbf{Performance Rectification}}   As for Performance Fairness, we rectify the valuation in distance and loss spaces simultaneously.  In FL scenarios, especially in medical ones, data distribution can be highly uneven among clients. For instance, some clients may have a large amount of data while others may have relatively little. In the distance space, we aim to avoid the unfair contribution of clients with larger data volumes on the global model. In loss space, the main purpose is to identify clients with poor performance through rectified by metrics loss and allocate more resources.


% scaling factor we rectify the scaling factor of each client . 

% We first calculate the weights of each client's feature vectors in distance space and loss space. 

In distance space, we calculate the scaling factor of L2-norm of the feature weight vector for all clients, denoted as $\left|\mathbf{g_{i, t}}\right|_2$. Then, calculate the sum of the L2-norms of the feature weight vectors for all clients, represented as $\sum_{i=1}^{\mathrm{N}}\left|\mathbf{g_{i, t}}\right|_2$. Combining these two formulas, we obtain the coefficient for the feature weight vector, i.e.,  $w_{i,\mathrm{\ Dis\ }}=\frac{\left|\mathbf{g_{i, t}}\right|_2}{\sum_{\mathrm{i}=1}^{\mathrm{N}}\left|\mathbf{g_{i, t}}\right|_2}$. As an indication of distance space, a gradient distance that is different from others may not be sufficient to fully rectify the contribution from a certain client to the FL performance fairness. 


To identify clients with poor performance, we further rectify in loss space. We use the square root of the ratio of the client's loss to the maximum loss as a weight coefficient for each client, i.e., $w_{i,\mathrm{\ loss\ }}=\frac{1}{2} \sqrt{\frac{\operatorname{loss}_i}{max\_{loss}}}$. Finally, the weights of each client in distance space and feature space are multiplied to obtain the weights of each client in performance fairness.


\paragraph{\textbf{Fairness Compensation}} We further rectifies the valuation of each client by comparing their above correlations with all other clients concerning both types of fairness, and then uses the rectified valuation as a weights to aggregate models.

\begin{equation}
\left\{\begin{array}{l}
w_{i, \text { Per }}=\sqrt{\frac{\operatorname{loss}_i}{\max l o s s}} \times \frac{\left\|\mathbf{g}_{\mathbf{i}, \mathbf{t}}\right\|_2}{2 \sum_{\mathrm{j}=1}^{\mathrm{N}}\left\|\mathbf{g}_{\mathbf{j}, \mathbf{t}}\right\|_2} \\
w_{i, \mathrm{Col}}= \frac{1}2 (w_{i, \mathrm{Dep}}+w_{i, \text { Dir }}) \\
 w_{i} = \lambda \times w_{i, \text { Per }} + (1-\lambda) \times w_{i, \mathrm{Col}}
\end{array}\right.
\end{equation}
where $\lambda$ is the weight to balance the Performance Fairness and Collaboration Fairness.


To ensure that all clients' weights are greater than a fairness threshold T and that the sum of all weights equals 1, we introduce a fairness compensation mechanism. Suppose the current smallest weight is $w_{min}$, if it is less than the threshold T, the weight compensation value is calculated as $\mathrm{compensation\ }=\frac{T-w_{min}}{N-1}$ where N is the number of clients. For each client i, the weight after compensation is:

\begin{equation}
w_i^\prime=\max\left(T,w_i+\mathrm{\ compensation\ } \right)
\end{equation}

where $w_i^\prime$ is the original weight calculated for client i, and T is the threshold. Finally, we normalize the weights so that their sum is 1, i.e., $w_i^{\text {final }}=\frac{w_i^\prime}{\sum_{j=1}^N w_j^\prime}$ where $w_i^{\mathrm{final\ }}$ is the final weight for client i.




\begin{algorithm}[t]
\caption{Our proposed method CMFL}
\begin{flushleft}
\textbf{Input:} Intra-graph; input samples. \\

\textbf{Output:} The final node embeddings $\mathbf{z}_v^r$, for $v \in \mathcal{V}$.\\
\end{flushleft}

\label{alg:FedGEM}
\begin{algorithmic}[1] %[1] enables line numbers
 
\FOR{$r=1...R$}

\STATE \text{Initialize} $\mathbf{z}_v^0 \leftarrow \mathbf{P}_{r} \cdot \mathbf{x}_v , \forall v \in \mathcal{V}$;
\FOR {$\Phi_h=\Phi_1...\Phi_H$}
%{$\Phi \in\left\{\Phi^{\mbox{intra}}, \Phi^{\mbox{inter}} \right\}$}
    \FOR{$k=1...K$}
        \FOR{$v \in \mathcal{V}_{\mbox{align}}$}
            \STATE Sample neighbors $\mathcal{P} = \mathcal{N}(v,\Phi_h)$;
        
            \STATE Aggregate neighbours $\mathbf{z}_{\mathcal{P}}^k \leftarrow \sum_{p \in \mathcal{P}} \mathbf{z}_{p}^{k-1}$;

            \STATE Calculate the concated node embeddings;
            \\ $\mathbf{z}_v^k \leftarrow \sigma\left(\mathbf{W}^k \cdot \left[\mathbf{z}_v^{k-1}|| \mathbf{z}_{\mathcal{P}}^k\right]\right)$;
            
            \STATE Aggregate negative nodes; \\ $\mathbf{z}_{\mathcal{R}(v)}^k \leftarrow \sum_{n \in \mathcal{F}(v)} \mathbf{z}_{n}^{k-1}$;
           
        \ENDFOR
    \ENDFOR
    \STATE $\mathbf{z}_{r,v}^{\Phi_h} \leftarrow \mathbf{z}_v^K,$ $\forall v \in \mathcal{V}_{align}$;

    \STATE Computes intra loss;
    
    \ENDFOR
    \STATE Back propagation and update intra-graph;
    
    \STATE Calculate attention weight and fuse semantic embeddings;

    
\ENDFOR
\STATE Compute total loss;


\STATE Back propagation and update inter-graph parameters;
\RETURN $\mathbf{z}_v^r$

\end{algorithmic}

\end{algorithm}




==> Section/4-experiments.tex <==
\section{Experiments}

\subsection{Experimental Setup}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
  \caption{Add caption}
    \begin{tabular}{c|cc|cc|cc|cc|cc}
        \toprule
    & \multicolumn{10}{c}{Task of HNSCC Segmentation} \\
    \cline{2-11}
    Method & \multicolumn{2}{c|}{AVG.} & \multicolumn{2}{c|}{No.1 (CT)} & \multicolumn{2}{c|}{No.2 (PET)} & \multicolumn{2}{c|}{No.3 (PT)} & \multicolumn{2}{c}{No.4 (PT)} \\
    \cline{2-11}
          & DICE ↑ & VOE↓  & DICE ↑ & VOE↓  & DICE ↑ & VOE↓  & DICE ↑ & VOE↓  & DICE ↑ & VOE↓ \\
    \hline
    Standalone & —     & —     & 0.6037 & 0.6293 & 0.6163 & 0.6204 & 0.5955 & 0.6081 & 0.5921 & 0.621 \\
    \hline
    Data-Centralized & 0.5641 & 0.5713 & —     & —     & —     & —     & —     & —     & —     & — \\
    \hline
    FedAvg & 0.6418 & 0.5832 & 0.6492 & 0.584 & 0.6368 & 0.5831 & 0.6385 & 0.5825 & 0.6426 & 0.583 \\
    \hline
    q-FedAvg & 0.6446 & 0.5691 & 0.6381 & 0.5665 & 0.6487 & 0.5701 & 0.6412 & 0.5693 & 0.6505 & 0.5702 \\
    \hline
    CGSV  & 0.6272 & 0.5889 & 0.616 & 0.5881 & 0.6223 & 0.5901 & 0.6342 & 0.5869 & 0.6362 & 0.5907 \\
    \hline
    CMFL (Ours.) & \textbf{0.6446} & \textbf{0.5691} & \textbf{0.6381} & \textbf{0.5665} & \textbf{0.6487} & \textbf{0.5701} & \textbf{0.6412} & \textbf{0.5693} & \textbf{0.6505} & \textbf{0.5702} \\

    
    \midrule
    
    & \multicolumn{10}{c}{Task of Whole-body FDG Segmentation} \\
    \cline{2-11}
    Method & \multicolumn{2}{c|}{AVG.} & \multicolumn{2}{c|}{No.1 (CT)} & \multicolumn{2}{c|}{No.2 (PET)} & \multicolumn{2}{c|}{No.3 (PT)} & \multicolumn{2}{c}{No.4 (PT)} \\
    \cline{2-11}
          & DICE ↑ & VOE↓  & DICE ↑ & VOE↓  & DICE ↑ & VOE↓  & DICE ↑ & VOE↓  & DICE ↑ & VOE↓ \\

    \hline
    Standalone & —     & —     & 0.8912 & 0.2681 & 0.8869 & 0.2706 & 0.8875 & 0.2719 & 0.8863 & 0.2744 \\
    \hline
    Data-Centralized & 0.9400  & 0.XX & —     & —     & —     & —     & —     & —     & —     & — \\
    \hline
    FedAvg & 0.7899 & 0.2807 & 0.4901 & 0.6025 & 0.8894 & 0.1736 & 0.8887 & 0.175 & 0.8907 & 0.1719 \\
    \hline
    q-FedAvg & 0.8161 & 0.2779 & 0.5421 & 0.5918 & 0.9068 & 0.1745 & 0.9072 & 0.1737 & 0.9082 & 0.1718 \\
    \hline
    CGSV  & 0.8153 & 0.2789 & 0.5387 & 0.5936 & 0.9071 & 0.1746 & 0.9077 & 0.1736 & 0.9076 & 0.1739 \\
    \hline
    CMFL (Ours.) & \textbf{0.8197} & \textbf{0.2679} & \textbf{0.5835} & \textbf{0.1882} & \textbf{0.8986} & \textbf{0.5548} & \textbf{0.8983} & \textbf{0.1887} & \textbf{0.8985} & \textbf{0.1882} \\

    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%






\textbf{Datasets.} In our experiments, we perform the model on two real-world datasets, which are described as follows:
\begin{itemize}
  \item \textbf{HNSCC} arises in the squamous cells lining the moist surfaces of the head and neck, including the mouth, nose, oropharynx, and larynx. The dataset contains clinical data and PT images of patients with head and neck squamous cell carcinoma who received radiotherapy. It includes DICOM segmentation of primary tumors and was divided into a training set of 58 cases and a verification set of 14 cases, with each case having 133 PET, CT, and SEG images. The training set contained 7,714 images and the verification set contained 1,862 images to ensure model generalization.
  \item \textbf{Whole-body FDG-PT} is a type of cancer that originates in one part of the body and spreads to other areas, forming multiple tumors throughout the body. Malignant lymphoma, melanoma, and NSCLC are common types of whole-body tumors. Malignant lymphoma affects the lymphatic system, melanoma is a skin cancer that can metastasize, while NSCLC is a type of lung cancer that can grow and spread quickly. The dataset contains anonymized original DICOM files and DICOM segmentation masks. It includes 1014 whole-body FDG-PT datasets from 2014 to 2018 at the University Hospital Tübingen, including 501 studies of patients with malignant lymphoma, melanoma, and NSCLC.
\end{itemize}


% 总结现有工作
\begin{figure}[t]
	\centering
     
	\subfigure[Distributions of different modalities]{\label{fig:head}
	\includegraphics[width=0.22\textwidth]{Section/Figure/whole-body_density_plot.pdf}}
	\subfigure[CT modality of different tumour]{\label{fig:head}
		
  \includegraphics[width=0.22\textwidth]{Section/Figure/Whole-body_type_density_plot.pdf}}
        \subfigure[Distributions of different modalities]{\label{fig:head}
		
  \includegraphics[width=0.22\textwidth]{Section/Figure/HNSCC_density_plot.pdf}}
  \subfigure[CT modality of different tumour]{\label{fig:head}
		
  \includegraphics[width=0.22\textwidth]{Section/Figure/HNSCC_type_density_plot.pdf}}
	
  \caption{Comparison of intensity distributions of }
	\label{fig:intro}
\end{figure}


\textbf{Data processing.} We preprocessed the case data in the original dataset in three steps (i) DICOM to NIfTI conversion: the original data was stored in DICOM (digital imaging and Communication) format, which is larger than NIfTI (Neuroimaging Informatics Technology Initiative) files. To facilitate subsequent data processing, we used the SimpleITK library to convert DICOM data into NIfTI format. (ii) Data Cleaning: some case data in the original dataset only had PET or CT ground truth, which we removed. Additionally, we excluded case data with a ground truth volume below a certain threshold (50\% of the original lesion ground truth) as the interception effect was not satisfactory, and we could not use these samples for training. (iii) Slice Extraction: After data cleaning, we extracted slices from PET and CT and converted them into 256PX by 256PX PNG format images.


% \begin{figure}[h]
% \begin{center}
%     \centering
%     \includegraphics[width=0.5\textwidth]{Section/Figure/.pdf}
% \caption{\textbf{Visualization of local image.}}
% \end{center}
% \end{figure}


% 总结现有工作
\begin{figure}[h]
	\centering
     
	\subfigure[Distributions of different modalities]{\label{fig:4q}
	\includegraphics[width=0.22\textwidth]{Section/Figure/mm_local_table.pdf}}
	\subfigure[Distributions of different modalities]{\label{fig:4b}
		\includegraphics[width=0.22\textwidth]{Section/Figure/mm_local_table.pdf}}
        \subfigure[CT modality of different tumour]{\label{fig:4c}
		\includegraphics[width=0.22\textwidth]{Section/Figure/mm_local_table.pdf}}
  \subfigure[CT modality of different tumour]{\label{fig:4d}
		\includegraphics[width=0.22\textwidth]{Section/Figure/mm_local_table.pdf}}
	
  \caption{Comparison of intensity distributions of }
	\label{fig:intro}
\end{figure}


\textbf{Evaluation metrics.} 

\paragraph{Segmentation Performance metrics.} Two metrics are utilized: (1) Sørensen–Dice (Dice)~\cite{}, which is a commonly used metric for evaluating the performance of image segmentation models. It is used to measure the similarity between the segmentation results produced by a model and the ground truth segmentation and is computed by:

\begin{equation}
\text{Dice} = 2 \cdot \frac{\left|Y \cap Y_{\text{pred}}\right|}{|Y| + |Y_{\text{pred}}|}
\end{equation}

where $Y$ and $Y_{\text{pred}}$ denote the ground truth and predicted segmentation masks, and $|Y|$ and $|Y_{\text{pred}}|$ represent the total number of voxels in the ground truth and predicted segmentation masks.


(2) Volume Overlap Error (VOE)~\cite{}, which is used to measure the degree of overlap between the segmentation output and the ground truth segmentation of a region of interest. A smaller VOE value indicates better segmentation performance. VOE is calculated as:

\begin{equation}
\operatorname{VOE} =1-\left|\frac{Y \cap Y_{pred}}{Y \cup Y_{pred}}\right|
\end{equation}

where $Y \cap Y_{pred}$ is the volume of the intersection between the predicted and ground truth segmentation, and $Y \cup Y_{pred}$ is the volume of the union of the predicted and ground truth segmentation.

% 形式：用一段话 描述就可以了
% 协作公平性指的是在全局模型的训练过程中，每个客户端都应该有机会参与训练并为全局模型做出贡献，以达到协作的目的。我们采用局部模型性能对比：计算 不同方法的最好客户端和最差客户端的差值
\paragraph{Collaboration Fairness metrics.}
% In federated learning, because the training data is distributed across multiple clients, you need to ensure that each client has the opportunity to participate in the training, rather than just a subset of clients contributing to the global model. This ensures that the global model better reflects the data distribution of individual clients, thus improving the performance and robustness of the model.
To assess collaborative fairness, we employ a local model performance comparison method that calculates the difference between the best and worst clients for different approaches~\cite{}. A smaller difference implies that each client has a chance to contribute to the global model, indicating higher collaborative fairness. In contrast, a larger difference suggests that some clients heavily influence the global model while others cannot effectively participate in the training, indicating unreliable collaborative fairness.

% To evaluate collaborative fairness, we use the local model performance comparison method, which calculates the difference between the best and worst clients of different methods. This difference can be used to measure the training quality of different clients. If the difference is small, it means that each client has the opportunity to contribute to the global model, indicating high collaborative fairness. On the contrary, if the difference is large, it means that some clients have a great influence on the global model, while other clients cannot effectively participate in the training, indicating that the fairness of the cooperation is low.


% 形式：一段话描述+公式表达
% Gini、雷夫指数 公式 + 描述公式的含义
\paragraph{Performance Fairness metrics.}
% a way is needed to measure the performance equity of federated learning.
We utilized two metrics to measure the performance fairness in FL: (1) Gini~\cite{}: A value closer to 0 signifies similar contributions from all participants, indicating fair performance, while a value closer to 1 implies disproportionate contributions from some participants, indicating unfair performance. The Gini is calculated using the following formula:

% (1) Gini coefficient~\cite{}, which is closer to 0 means that all participants have similar contributions to the model, indicating a fair performance, while a Gini coefficient closer to 1 indicates that some participants have disproportionately large contributions, indicating an unfair performance. The formula for calculating the Gini coefficient as follow:

% Because of the uneven distribution of data among participants, this may result in contributions from some participants having an impact on the quality of the global model. 

% range from 0 to 1, where 0 represents perfect equality and 1 represents perfect inequality. A Gini coefficient 

% ranges from 0 to 1, with 0 being perfect equality and 1 being perfect inequality. If the Gini coefficient is close to 0, it means that all participants have similar contributions to the model quality and the performance is fair. If the Gini coefficient is close to 1, it indicates that the contribution of some participants is too large and the performance is not fair.




\begin{equation}
\text{Gini} = 1-2 \cdot \frac{\sum_{i=1}^{n} w_{i} \sum_{j=1}^{i} d_{j}}{n \sum_{i=1}^{n} w_{i} d_{i}}
\end{equation}


where $n$ represents the number of clients, $w_i$ denotes the sample weight of the $i$-th client, and $d_i$ is the $i$-th client's segmentation performance, sorted in ascending order.


% In this formula, $\sum_{j=1}^i d_{j}$represents the sum of Dice coefficients of the first $i$clients after Dice coefficient sorting, and $\sum_{i=1}^n w_{i}d_{i}$represents the sum of Dice coefficient weighted sum of all clients after Dice coefficient sorting.

(2) Relative Fractional Accuracy (RFA)~\cite{} measures each client's contribution and overall performance. A higher RFA indicates more balanced contributions and better algorithm performance. RFA is calculated as follows:

% , which is used to measure the contribution of each client and the overall performance. The higher the RFA index is, the closer the contribution of each client is, and the better the overall algorithm performance is. The calculation of RFA is as follow:

\begin{equation}
\text{RFA} = \frac{1}{n} \cdot \sum_{i=1}^{n} \frac{w_{i}}{\bar{w}} \frac{d_{i}- \bar{d} }{ \bar{d} }
\end{equation}

where $n$ represents the number of clients, $w_i$ denotes the sample weight of the $i$-th client, $\bar{w}$ is the average sample weight, $d_i$ represents the segmentation performance of the $i$-th client, and $\bar{d}$ is the average segmentation performance.

% where $n$ represents the number of clients, $w_i$ represents the weight of the $i$ client, $\bar{w}$ represents the average weight of all clients, $d_{i}$ represents the dice of the $i$  client, and $\bar{d}$ represents the average dice of all clients.






\begin{figure*}[ht]
\begin{center}
    \centering
    \includegraphics[width=0.9\textwidth]{Section/Figure/mm_line.pdf}
\caption{\textbf{Convergence analysis in terms of validation Dice score with the different number of communication rounds.}}
    \label{fig:FedGEM_e}
\end{center}
\end{figure*}

% 参考我发你的pdf里的内容
\paragraph{\textbf{Baselines.} } We conducted a comparative analysis of our methodology against five baseline methods, including: 1) Standalone, a method involving local training and evaluation on the client side; 2) Centralized, a centralized training approach; 3) FedAvg, a commonly used federated learning algorithm; 4) CGSV, a method for estimating Shapley values, which promotes collaboration fairness through cosine similarity; and 5) q-FedAvg, a method that achieves performance fairness for worse-performing clients by implementing weighted averaging, with an optimal proportion of q=0.5. Based on this, we further compared our approach with these baseline methods.


\paragraph{\textbf{Implementations.}} Following the experimental settings of previous works, we conducted our federated learning experiment with four clients. The network was trained for 200 epochs with a batch size of 4, using the Adam optimizer with a momentum value between 0.9 and 0.999 and an initial learning rate of 1e-4. The Adam optimizer with momentum gradient descent is an adaptive learning rate adjustment mechanism. \textcolor{red}{weight and so on }
% 增加涉及到的权重，\lamnda 表示 weight，使用余弦和皮尔森和欧式相似函数等等






\subsection{Experimental Results}

% 这部分等全表的跑完，再一起讨论下再写
% 形式：总结 + 现象说明 (表1 + 图2) 。可以先写现象说明，就是介绍实验结果，和其他方法相比，分别大于多少等等。再给出一个结论。
% 最后 调换一下顺序，先放结论在前面，再写现象说明
\textcolor{red}{\textbf{Segmentation performance.}}

\textcolor{red}{Our results led to three key observations. First, ....... Specifically, we observed that (Figure).  Second, we highlight the effectiveness (Table). Third,(Figure). }


% 形式：总结 + 现象说明 (表2) 。可以先写现象说明，就是介绍实验结果，和其他方法相比，分别大于多少等等。再给出一个结论。
% 然后调换一下顺序，先写结论，再写现象说明
\textcolor{red}{\textbf{Collaboration Fairness.} }




% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{c|c|c|c|c}
    \toprule
    Task  & \multicolumn{2}{c|}{\makecell{Task of HNSCC \\ Segmentation}} & \multicolumn{2}{c}{\makecell{Task of Whole-body \\ FDG Segmentation}} \\    
    \hline
    Metric & $\triangle$. DICE ↓ & $\triangle$. VOE ↓ & $\triangle$. DICE ↓ & $\triangle$. VOE ↓ \\
    \hline
    FedAvg & 0.5110 &0.3517 & 0.4686 & 0.4615 \\
    \hline
    q-FedAvg &0.6421 & 0.4308 & 0.4572 & 0.4585 \\
    \hline
    CGSV  &  0.5826 & 0.4114 & 0.4557 & 0.4559 \\
    \hline
    CMFL (Ours.) & \textbf{ 0.4243} & \textbf{ 0.4241} & \textbf{0.4117} & \textbf{0.4129} \\

    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%



% 形式：总结+现象说明 (表3)。可以先写现象说明，就是介绍实验结果，和其他方法相比，分别大于多少等等。再给出一个结论。
% 然后调换一下顺序，先写结论，再写现象说明
\textcolor{red}{\textbf{Performance Fairness.} }


\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{c|c|c|c|c}
    \toprule
    Task  & \multicolumn{2}{c|}{\makecell{Task of HNSCC \\ Segmentation}} & \multicolumn{2}{c}{\makecell{Task of Whole-body \\ FDG Segmentation}} \\
    \hline
     Metric & Gini↓ & RFA ↑ & Gini↓ & RFA ↑ \\
    \hline
    FedAvg & 0.2800  & 0.9995 & 0.2100  & 0.8569 \\
    \hline
    q-FedAvg & 0.2700  & 0.9983 & 0.1700  & 0.8651 \\
    \hline
    CGSV  & 0.3000   & 0.9985 & 0.1700  & 0.8652 \\
    \hline
    CMFL (Ours.) & \textbf{0.2900} & \textbf{0.9989} & \textbf{0.1600} & \textbf{0.8758} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

\subsection{Ablation Study} We further conduct in-depth analytical studies to

\textbf{Analysis of Contribution of Each Component.} We further conduct the ablation study for ....


% 参考之前发的CVPR23的方法的写作
\textbf{Analysis of Convergence speed.} 
The convergence rate is a crucial performance index in FL algorithms.       Aggregating local models from multiple clients into a global model while protecting data privacy is achieved through communication rounds involving multiple clients participating in model updates.     Comparing convergence rates among FL methods involves observing client scores for each communication round.       A method converging to higher performance and faster speed indicates a better convergence rate.       We utilize validation Dice scores across clients per communication round for various methods.      We applied the Locally Weighted Scatterplot Smoothing to smoothen the curves, better highlighting the overall trend.    Our aggregation method effectively enhances the global model's convergence rate, achieving higher performance levels more rapidly than comparable methods.

% Convergence rate is one of the important indexes to measure the performance of federated learning algorithm. In federated learning, since data is distributed on multiple clients, it is necessary to aggregate the local model of each client to obtain a global model on the premise of protecting data privacy. The aggregation process is accomplished through a communication round, which typically involves multiple clients participating in model updates.
% When comparing the convergence rates of different federated learning methods, the client score for each communication turn can be observed. If the curve of a method converges to higher performance and faster speed, it indicates that the method has better convergence rate. We first show the validation Dice score across clients per communication round for different FL methods. As shown in Figure 3, the contribution value-based aggregation method we used can effectively improve the convergence rate of the global model. Our approach calculates the average verification dice score between clients on each communication turn and achieves higher performance levels faster than other comparable FL approaches. Because our contribution-based aggregation approach utilizes gradient information from different clients, it facilitates global model optimization across the overall data distribution. The observations confirm our theoretical analysis that using contribution estimates to aggregate the model in FL helps promote convergence.



\begin{figure}[h]
\begin{center}
    \centering
    \includegraphics[width=0.45\textwidth]{Section/Figure/mm_images (1).pdf}
\caption{\textbf{Visualization of image.}}
\end{center}
\end{figure}






==> Section/5-conclusion.tex <==
\section{CONCLUSIONS}

 Density map is a visual method to measure the similarity between different data by looking at the cross area product. In the case of different modes, the density map shows great unbalance. Within the same mode, there is relatively little imbalance between different diseases.This may lead to poorer performance for clients with fewer data or larger differences in data distribution;
